Coherent collapse of a dipolar Bose-Einstein condensate for different trap geometries

We experimentally investigate the collapse dynamics of dipolar Bose- Einstein condensates of chromium atoms in different harmonic trap geometries, from prolate to oblate. The evolutions of the condensates in the unstable regime are compared to three-dimensional simulations of the Gross-Pitaevskii equation including three-body losses. In order to probe the phase coherence of collapsed condensates, we induce the collapse in several condensates simultaneously and let them interfere.

==> Makefile <==
##################################################
## Makefile zum erstellen von LaTeX Dokumenten
##################################################


#Name der erzeugten Datei (ohne Extension)
NAME = CoherentCollapse_Preprint
LITERATURVERZEICHNIS= 
TEXFILES = *.tex	 	        # Binde alle LateX-Dateien ein
PICTURES = #./fig/* #./mathematica/*	# Pfad zu den Bildern
STYLEFILES = 


TablesOfContens = $(NAME).toc
TableOfFigures  = #$(NAME).lof
TableOfTables   = #$(NAME).lot
INHALTESVERZEICHNISSE = $(TablesOfContens) $(TableOfFigures) $(TableOfTables)


### Für Verweise (Kapitel, Gleichungen, ...)
# .aux: von Latex erzeugt; beinhaltet alle Verweise
# .bib: verwendet von Bibtex um die Verweise aus den .aux-Dateien aufzulösen
# .bst: Styl-Datei: wie sollen die Verweise im .dvi aussehen
# .blg: Log-Datei von Bibtex
# .bbl: output aus Bibtex. Beim nächsten Latex-Lauf werden diese eingebunden
#       Latex muss zwei (manchmal drei) mal laufen!!!
# .idx: von Latex erzeugt; beinhaltet alle Indexe
AUXFILES = *.aux 		# zu jeder Datei gibt es eine .aux-Datei
BIBTEXFILES = $(NAME).bib 	#$(NAME).bbl 
INDEXFILES = # $(NAME).idx  	#$(NAME).ist $(NAME).ind $(NAME).glo $(NAME).gls





## Nützliches Programm zur Fehlersuche: 
## * auctex
##   Strg+c, Strg+c     kompilieren
##   Strg+c, `          Fehler anzeigen
##   Strg+c, Strg+c     dvi anzeigen
## * lacheck
##   in Emacs: Alt+x compile
##             lacheck DATEINAME.tex
##             Mittlere Maustaste springt zum Fehler


#### ÄNDERUNGEN: ###################################################
# 05-08-22: * BibTeX wird nur ausgeführt, falls dies notwendig ist
#	      Unterdrücke unwichtiges aus BibTeX (benutze grep -v)
#             Warnings werden ganz zum Schluß herausgeschrieben
# 05-08-30: * LaTeX gibt nicht mehr alles auf den Bildschirm aus, sondern
#	      nurnoch Fehlermeldungen
#           * Warnungen von BibTeX werden immer angezeigt
# 05-12-03  * Abhängigkeiten von dvi und BibTeX richtig gemacht
# 06-01-25  * BibTeX wird vor LaTeX ausgeführt, so dass Änderungen im Literaturverzeichnis
# 	      sofort eingearbeitet werden
# 06-11-10  * mpage erzeugt übersicht über Dokument -> für Präsentationen (talks)
# 06-11-20  * Index hinzugefügt (NICHT getestet!!!)


####################################################################
# Noch zu machen:
# * pdflatex Option 
# * make ci         ... checkt in Revisioncontrol-System ein
# * Falls Datei .tof oder .bbl nicht vorhanden ist, dann bricht Programm ab. Deshalb habe ich
#   leere Targets mit diesem Name (ganz am Ende des Makefiles) erstellt. Dies muss geändert werden
# * Falls in $(NAME).log ein Ausrufe Zeichen ganz zu Beginn einer Zeile steht, dann hat LaTeX einen
#   Fehler gemacht. Wie kann man mit grep dies Zeilenanfang überprüfen???




###################################################################
## Diese Einstellungen sind soweit gut (brauche nichts zu ändern):
###################################################################
## Wo sind die Befehle definiert -- das Programm sucht selbst.
## Diese Programme müssen installiert sein und gefunden werden
BIBTEX=`which bibtex`		#/usr/bin/bibtex
CONVERT2PDF=`which 2pdf`	# dies ist kein Standardprogramm -> benutze convert
DVIPDF=`which dvipdfm`		#/usr/bin/dvipdfm
DVIPS=`which dvips`  		#/usr/bin/dvips
EMACS=`which emacs`
GREP=`which grep`
GV=`which gv`			#/usr/X11R6/bin/gv
LATEX=`which latex` 		#/usr/bin/LaTeX
MAKEINDEX=`which makeindex`
LATEX2HTML=`which latex2html`	#/usr/bin/latex2html
PSBOOK=`which psbook`		#/usr/bin/psbook
PDFLATEX=`which pdflatex`	#/usr/bin/pdflatex
PSLATEX=`which pslatex`		#/usr/bin/pslatex
PSNUP=`which psnup`		#/usr/bin/psnup
PS2PDF=`which ps2pdf`		#/usr/bin/ps2pdf
PS2PS=`which pstops`		#/usr/bin/pstops
PSRESIZE=`which psresize`	#/usr/bin/psresize
RM=`which rm` -f		#/bin/rm
SED=`which sed`			#/usr/bin/sed
TAR=`which tar`			#/bin/tar
THUMBPDF=`which thumbpdf`
TOUCH=`which touch`		#/usr/bin/touch
# PDFVIEWER="open -a  PDFView.app" # MAC
PDFVIEWER="open -a skim.app" # MAC
XPDF=`which xpdf`		#/usr/bin/xpdf
ACROREAD="acroread"
PSPRESENT=`which pspresent`	#/home/jjj/bin/pspresent
#MPAGE=`which mpage` # nicht installiert
XDVI=`which xdvi`
XDVIK=`which xdvik`
OPEN=`which open `		#für Apple




### OPTIONEN für Programme
DVIPDFFLAGS=-p a4 -z 9          # -z compression_level (9 ist Maximal)
DVIPSFLAGS=-Ppdf -GO -D 600 	# -Ppdf -GO um keine Bitmap-Schrift zu bekommen
PDFoptionen=-remote $(XPDF-REMOTENAME)
PS2PSFLAGS='4:0L(21cm,0)+1L(21cm,14.85cm),2R(0,29.7cm)+3R(0,14.85cm)'
PS2PDFFLAGS='-dPDFSETTINGS=/prepress -DEncodeColorImage=false' # 06-11-11: Kofler S.317 optimale Qualität
XPDF-REMOTENAME=Diplomarbeit
XPDF-praesentation=-fullscreen



# Da dies der erste Punkt ist, kann man ihn mit make aufrufen:
# Aufruf mit 'make' (ohne Option)
.PHONY : default
default:
	@ ${MAKE} pdf


##################################################
## define the pure programms (just do what the name says)
##################################################
.PHONY : LATEX
LATEX:  $(TEXFILES) $(PICTURES) $(INHALTESVERZEICHNISSE) $(BIBTEXFILES) $(INDEXFILES)
	@ ${MAKE} MakeLatex


.PHONY : PSLATEX
PSLATEX: $(TEXFILES) $(PICTURES) $(INHALTESVERZEICHNISSE) $(BIBTEXFILES) $(INDEXFILES)
	@ ${MAKE} MakePSlatex

.PHONY : PDFLATEX
PDFLATEX: $(TEXFILES) $(PICTURES) $(INHALTESVERZEICHNISSE) $(BIBTEXFILES) $(INDEXFILES)
	@ ${MAKE} MakePDFlatex


.PHONY : BIBTEX
BIBTEX: $(AUXFILES) $(BIBTEXFILES)
	@ ${MAKE} MakeBibtex

.PHONY : MAKEINDEX
MAKEINDEX: $(TEXFILES) $(INDEXFILES)
	@ ${MAKE} MakeBibtex


.PHONY : WARNINGS
WARNINGS: $(NAME).log
	@ ${MAKE} MakeWarnings


.PHONY : UNDEFREF
UNDEFREF: $(NAME).log
	@ ${MAKE} MakeUndefinesReferences


##################################################
## DVI: define the program which is normally used to produce a dvi
##################################################
.PHONY : dvi
$(NAME).dvi: $(TEXFILES) $(PICTURES) $(BIBTEXFILES)
	@ if [ -e $(NAME).blg ]; then \
	   ${MAKE} BIBTEX; \
	  fi
	@ ${MAKE} LATEX
	@ if [ ! -e $(NAME).blg ]; then \
	   ${MAKE} BIBTEX; \
	  fi
	@ ${MAKE} WARNINGS		# LaTeX Warnungen
	@ ${MAKE} UNDEFREF		# undefined references
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $XDVIK $(NAME).dvi &"


##################################################
## PS: define the program which is normally used to produce a ps
##################################################
.PHONY : pslatex
pslatex: $(TEXFILES) $(PICTURES) $(INHALTESVERZEICHNISSE) $(BIBTEXFILES) $(INDEXFILES)
	@ echo "Starte psLaTeX ....."
	@ echo "Erstelle die Datei $(NAME).ps ....."
	@ ${MAKE} PSLATEX
	@ echo "LaTeX ohne Fehler beendet."
	@ ${MAKE} BIBTEX		# rufe BIBTEX auf
	@ ${MAKE} WARNINGS
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $(GV) $(NAME).ps &"


.PHONY : ps
$(NAME).ps ps: $(NAME).dvi 					#ruft den Punkt dvi auf
	@ ${MAKE} 2ps


#falls dvi bereits vorhanden
.PHONY : 2ps
2ps:	
	@ # Falls dvi-Datei nicht vorhanden, erstelle sie
	@ if [ ! -e $(NAME).dvi ];\
	  then \
		${MAKE} $(NAME).dvi ;\
	  fi
	@ echo "#############################################"
	@ echo "## PS"
	@ echo "#############################################"
	@ echo "Erstelle die Datei $(NAME).ps ....."
	@ $(DVIPS) $(DVIPSFLAGS) $(NAME).dvi &> /dev/null # Umleitung nach /dev/null funkioniert nicht ???
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $(GV) $(NAME).ps &"


##################################################
## PDF: define the program which is normally used to produce a pdf
## Muss in der header-Datei eine Vektor-Schrift auswählen, damit es perfekt aussieht
##################################################
.PHONY : pdflatex
pdflatex: $(TEXFILES) $(PICTURES) $(INHALTESVERZEICHNISSE) $(INDEXFILES) #$(BIBTEXFILES)
	@ echo "Benutze pdfLaTeX."
	@ ${MAKE} PDFLATEX
	@ ${MAKE} BIBTEX		# nicht getetet
	@ ${MAKE} WARNINGS		# nicht getetet
	@ echo ""
	@ echo "Vorschlag: "
	@ if [ `uname` = Darwin ]; then \
		echo "   $(PDFVIEWER) $(NAME).pdf &"; \
	  else \
		echo "   $(XPDF) $(XPDFoptionen) $(NAME).pdf &";\
	  fi


.PHONY : pdf
$(NAME).pdf pdf: $(NAME).ps
	@ ${MAKE} ps2pdf


# falls dvi bereits vorhanden
.PHONY : 2pdf
2pdf:
	@ # ps-Datei existiert nicht
	@ #   -> Existiert dvi-Datei? Falls ja, so erstelle erstelle eine ps-Datei
	@ #                           Falls nein, so erstelle erste eine dvi-Datei und
	@ #                              anschließend eine ps-Datei
	@ # Falls eine ps-Datei existiert, so erstelle eine pdf-Datei aus der ps-Datei
	@ if [ ! -e $(NAME).ps ];\
	  then \
		if [ ! -e $(NAME).dvi ];\
	  	then \
			${MAKE} $(NAME).ps  ;\
		else \
			${MAKE} 2ps ;\
		fi;\
	  fi
	@ ${MAKE} ps2pdf 


.PHONY : ps2pdf
ps2pdf:
	@ echo "Erzeuge eine pdf-Datei aus der Datei $(NAME).ps"
	@ echo "Dies kann einen Moment dauern....."
	@ $(PS2PDF) $(PS2PDFFLAGS) $(NAME).ps
	@ echo ""
	@ echo "Vorschlag: "
	@ if [ `uname` = Darwin ]; then \
		echo "   $(PDFVIEWER) $(NAME).pdf &"; \
	  else \
		echo "   $(XPDF) $(XPDFoptionen) $(NAME).pdf &";\
	  fi


.PHONY : dvi2pdf
dvi2pdf:
	@ echo "***** ACHTUNG:"
	@ echo -n "Die Ersetzung in bildern mittels psfrag wird nicht unterstützt"
	@ read muell
	@ echo "#############################################"
	@ echo "## PDF"
	@ echo "#############################################"
	@ echo "Starte dvipdfm ....."
	@ $(DVIPDF) $(DVIPDFFLAGS) $(NAME).dvi &> /dev/null 
	@ echo ""
	@ echo "Vorschlag: "
	@ if [ `uname` = Darwin ]; then \
		echo "   $(PDFVIEWER) $(NAME).pdf &"; \
	  else \
		echo "   $(XPDF) $(XPDFoptionen) $(NAME).pdf &";\
	  fi


.PHONY : thumbpdf
thumbpdf: $(NAME).pdf
	@ echo "##################################################"
	@ echo "## Thumbnails"
	@ echo "##################################################"
	@ echo "Erstelle ein kleines Bild von jeder Seite....."
	@ $(THUMBPDF) --modes=ps2pdf $(NAME).pdf # erstelle Thumbnails in $(NAME).tpt
	@ ${MAKE} pdf


##################################################
## HTML: define the program which is normally used to produce a html
##################################################
.PHONY : 4html
4html:  $(NAME).dvi
	@ htlatex.bat $(NAME).tex "xhtml,2,fn-in,NoFonts,fonts,graphics-,sections+,next"
	@ echo "Vorschlag:"
	@ echo "     opera $(NAME).tex"

.PHONY : 2html
2html:
	@ echo "Starte latex2html ....."
	@ $(LATEX2HTML) $(NAME).tex
	@ echo ""
	@ echo "Vorschlag:"
	@ echo "     opera $(NAME).tex"




# für doppelseitigen Text
.PHONY : psnup
psnup:
	@ if [ ! -e $(NAME).ps ]; \
	  then \
		${MAKE} $(NAME).ps ;\
	  fi
	@ echo "Erstelle ein Doppelsitiges Dokument ....."
	@ $(PSNUP) -pa4 -2 $(NAME).ps $(NAME)2.ps
	@ echo "Doppelseitige Datei gespeichert in $(NAME)2.ps"
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $(GV) $(NAME)2.ps &"


.PHONY : a5book
a5book: # erstellt ein a5-Buch aus a4-Seiten (dante Seite 160)
	@ echo "Erstelle dvi-Datei ....."
	@ $(DVIPS) -o tmp-a4.ps $(NAME).dvi &> /dev/null 
	@ echo "Korrigiere Papiergröße von a4 nach a5 ....."
	@ $(PSRESIZE) -Pa4 -Pa5 tmp-a4.ps tmp-a5.ps &> /dev/null 
	@ echo "Sortieren der Seiten"
	@ echo "  16 Seiten ergeben 4 Bögen (doppelseitig und gefaltet)....."
	@ $(PSBOOK) -s16 tmp-a5.ps tmp-sorted.ps  &> /dev/null 
	@ echo "Zusammenfassen von 4 Seiten auf einem DIN A4-Blatt....."
	@ $(PS2PS) '$(PS2PSFLAG)' tmp-sorted.ps $(NAME)-a5book.ps  &> /dev/null 
	@ echo "Aufräumen ....."
	@ $(RM) tmp-a4.ps tmp-a5.ps tmp-sorted.ps 
	@ echo "Die Datei $(NAME)-a5book.ps wurde erzeugt."
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $(GV) $(NAME)-a5book.ps &"

.PHONY : mpage
mpage :
	@ echo "Mpage ist noch nicht installiert"
	@ exit;
	@ echo "Erstelle eine Übersicht ....."
	@ $(MPAGE) -64 $(NAME).ps > $(NAME)_a64.ps
	@ echo ""
	@ echo "Vorschlag: "
	@ echo "   $(GV) $(NAME)-a5book.ps &"

# xpdf neu laden, falls Änderungen am Dokument vorgenommen wurden
.PHONY : reload reloadxpdf
reload reloadxpdf:
	@ echo "Reload xpdf.."
	@ps -af | grep "$(XPDF) $(XPDFoptionen)" | grep -q -v "grep" && -remote $(XPDF) $(XPDFoptionen) -reload


.PHONY : eps2pdf
eps2pdf:
	@ echo "Mache aus den .eps-Bildern pdfs....."
	@ # Wandle alle .eps in .pdf um.
	@ # Dazu schaue ich zunächst, ob pdf bereits existiert
	@ for bild in `find -name *.eps`; do \
		pdf=$${bild%.eps}.pdf;\
		if [ ! -e $$pdf ]; then \
			$(CONVERT2PDF) $$bild;\
		fi;\
	  done;


# falls BibTeX erzwungen werden soll
.PHONY : bib
bib:    
	@ $(BIBTEX) $(NAME)


ARCHIVDATEI=$(NAME)_$$(date "+%y_%m_%d")
.PHONY : archiv tar backup tgz
$(NAME).tgz archiv backup tar tgz: dvi $(TEXFILES) Makefile $(PICTURES) $(STYLEFILES) $(LITERATURVERZEICHNIS)
	@ echo "##################################################"
	@ echo "## Erstelle Archiv ....."
	@ echo "##################################################"
	@ cp $(NAME).dvi $(NAME).save # damit es beim clean nicht gelöscht wird
	@ ${MAKE} cleanBackup
	@ mv $(NAME).save $(NAME).dvi
	@ mkdir $(ARCHIVDATEI)
	@ mkdir $(ARCHIVDATEI)/fig/
	@ cp -r $(TEXFILES) Makefile $(STYLEFILES) $(LITERATURVERZEICHNIS) $(NAME).dvi \
		$(ARCHIVDATEI)
	@ cp -r $(PICTURES) $(ARCHIVDATEI)/fig/.
	@ $(TAR) czf $(ARCHIVDATEI).tgz $(ARCHIVDATEI)
	@ $(RM) -r $(ARCHIVDATEI)
	@ echo Archivdatei ist $(ARCHIVDATEI).tgz
	@ echo "Vorschlag"
	@ echo "   cp $(ARCHIVDATEI).tgz /media/usbdisk/."


.PHONY : tar-all
tar-all: $(TEXFILES) $(PICTURES) Makefile $(LITERATURVERZEICHNIS) $(STYLEFILES)
	@ echo "Erstelle Archiv ....."
	@ if [ -e $(NAME).ps -a -e $(NAME).pdf ]; \
	  then \
		$(TAR) czf $(NAME)_$$(date "+%y_%m_%d").tgz \
	 	$(TEXFILES) $(PICTURES) Makefile $(STYLEFILES) $(LITERATURVERZEICHNIS) $(BACKUPFILES) \
	 	$(NAME).ps $(NAME).pdf ;\
		echo "Archivdatei ist $(NAME)_$$(date "+%y_%m_%d").tgz";\
	  elif [ -e $(NAME).ps ];\
	  then \
		$(TAR) czf $(NAME)_$$(date "+%y_%m_%d").tgz \
	 	$(TEXFILES) $(PICTURES) Makefile $(STYLEFILES) $(LITERATURVERZEICHNIS) $(BACKUPFILES) \
	 	$(NAME).ps ;\
		echo "WARNUNG: es ist keine pdf-Datei enthalten";\
		echo "Archivdatei ist $(NAME)_$$(date "+%y_%m_%d").tgz";\
	  elif [ -e $(NAME).pdf ];\
	  then \
		$(TAR) czf $(NAME)_$$(date "+%y_%m_%d").tgz \
	 	$(TEXFILES) $(PICTURES) Makefile $(STYLEFILES) $(LITERATURVERZEICHNIS) $(BACKUPFILES) \
	 	$(NAME).pdf ;\
		echo "WARNUNG: es ist keine ps-Datei enthalten";\
		echo "Archivdatei ist $(NAME)_$$(date "+%y_%m_%d").tgz";\
	  else \
		${MAKE} tar ;\
		echo "WARNUNG: es ist keine ps-Datei enthalten";\
		echo "WARNUNG: es ist keine pdf-Datei enthalten";\
	  fi


# Um stendig ein aktuelles dvi zu erhalten
.PHONY : loop
loop:
	@ echo "Starte Loop ....."
	@ while true; do ${MAKE} -q || ${MAKE}; sleep 1; done


# öffnet die Masterdatei
tex:
	@ $(EMACS) $(NAME).tex &


# zum Betrachten der output-Datei
.PHONY : gv
gv:
	@ echo "Starte gv....."
	@ # Muss & durch $ schützen
	@ if [ -e $(NAME).ps ]; \
	  then \
		$(GV) $(NAME).ps $& ; \
	  else \
		echo "$(NAME).ps existiert nicht.";\
	  fi

# Bildschirm-Präsentation von PS-Datei (sehr schnell) - talks
pspresent:
	@ echo "Starte 'iRed Lite' für Apple-Fernbedienung ..."
	@ RemoteControl
	@ $(PSPRESENT) $(NAME).ps &

#  Bildschirm-Präsentation von PDF-Datei (sehr schnell) - talks
pdfpresent:
	@ echo "Starte 'iRed Lite' für Apple-Fernbedienung ..."
	@ RemoteControl
	@ # $(XPDF) $(XPDF-praesentation) $(NAME).pdf &
	@ $(ACROREAD) $(NAME).pdf &



.PHONY : xpdf
xpdf:
	@ echo "Starte xpdf....."
	@ if [ -e $(NAME).pdf ]; \
	  then \
		$(XPDF) $(XPDFoptionen) $(NAME).pdf $& ;\
	  else \
		echo "$(NAME).pdf existiert nicht.";\
	  fi

.PHONY : BibDesk
BibDesk:
	@ echo "Dies wurde nicht getestet. Mache zunächst eine Sicherheitskopie von  $(LITERATURVERZEICHNIS)"
	@ echo "Sicherheitskopie darf nicht automatisiert werden, weil sonst sinnlos"
	@ echo "Führe dies nicht zu oft aus (nur bei absolut FERTIGER Arbeit)"
	@ echo "Anschließend:    make BibDeskForce"
	@ echo "Abbruch"
	@ exit
literaturefile: # gehoert eigentlich zu BibDeskForce
	@ sed 's/ä/{"a}/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/ö/{"o}/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/ö/{"o}/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/ü/{"u}/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/\<C3\>\<97\>/$$\times$$/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/<SUP>/$$^{/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's#</SUP>#}$$#g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/<CE><BC>/$$\mu$$/g' $(LITERATURVERZEICHNIS) > tmp.muell ; mv tmp.muell  $(LITERATURVERZEICHNIS)
BibDeskForce:
	@ ### Dies erleichtert die Fehlersuche, weil es zentriert ist: siehe MACRO in bst-Datei (style-file fuer BibTeX)
	@ sed 's/journal =/Journal =/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/journal=/Journal =/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/pra/PRA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/pre/PRE/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/pla/PLA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/prl/PRL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/ajp/AJP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ ###
	@ sed 's/Am. J. Phys./AJP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Eur. Phys. Lett./EPL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/J. App. Phys./JAP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Opt. Comm./OC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Opt. Lett./OL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Lett. A/PLA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rep./PRep/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. A/PRA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. B/PRB/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. C/PRC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. D/PRD/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. E/PRE/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys. Rev. Lett./PRL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHN)
	@ sed 's/Rev. Mod. Phys./RMP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS
	@ sed 's/Rev. Sci. Inst./RSI/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)IS)
	@ ###
	@ sed 's/Americal Journal of Physics/AJP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/European Physical Letters/EPL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Journal of Applied Physics/JAP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Optics Communications/OC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Optics Letters/OL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Letters A/PLA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physics Reports/PRep/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review A/PRA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review B/PRB/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review C/PRC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review D/PRD/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review E/PRE/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Physical Review Letters/PRL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Review of Modern Physics/RMP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS
	@ sed 's/Review of Scientific Instrumts/RSI/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS))
	@ ###
	@ sed 's/Am J Phys/AJP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Eur Phys Lett/EPL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/J App Phys/JAP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Opt Comm/OC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Opt Lett/OL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Lett A/PLA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rep/PRep/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev A/PRA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev B/PRB/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev C/PRC/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev D/PRD/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev E/PRE/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Lett A/PLA/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Phys Rev Let/PRL/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Rev Mod Phys/RMP/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/Rev Sci Ins/RSI/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ ###
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/nature/Nature/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/nat/Nature/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/science/Science/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/arxiv/arXiv/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/Arxiv/arXiv/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/ArXiv/arXiv/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Journal =" $(LITERATURVERZEICHNIS) | sed 's/ARXIV/arXiv/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ ###
	@ sed 's/month =/Month =/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ sed 's/month=/Month =/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)	
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Januar/Jan/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Februar/Feb/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/März/Mar/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/April/Apr/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Mai/May/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Juni/Jun/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Juli/Jul/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/August/Aug/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/September/Sep/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Oktober/Oct/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/November/Nov/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/Dezember/Dec/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/January/Jan/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/February/Feb/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/March/Mar/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/June/Jun/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/July/Jul/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/December/Dec/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/jan/Jan/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/feb/Feb/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/mar/Mar/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/may/May/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/apr/Apr/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/jun/Jun/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/jul/Jul/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/aug/Aug/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/sep/Sep/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/nov/Nov/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ grep "Month =" $(LITERATURVERZEICHNIS) | sed 's/dec/Dec/g' $(LITERATURVERZEICHNIS) > tmp.muell; mv tmp.muell  $(LITERATURVERZEICHNIS)
	@ $(RM) tmp.muell

.PHONY : clean		# falls eine Datei 'cleanBackup' heißt, so verschluckt sich make ansonsten
clean:
	@ echo "Lösche unwichtige Dateien ....."
	@ $(RM) *.aux			# Querverweise
	@ $(RM) *~			# Backups von emacs
	@ $(RM) *.bak			# Backups von xfig
	@ $(RM) *.tmp			# temporäre Dateien
	@ $(RM) *.log			# LaTeX-Ausgabe beim compilieren
	@ $(RM) *.nav
	@ $(RM) *.out
	@ $(RM) *.snm
	@ $(RM) *.blg			# vorangegangener BibTeX-Aufruf
	@ $(RM) *.ilg			# vorangegangenes Indexverzeichnis
# 	@ $(RM) *.cls			# Befehlsdefinitionen
	@ $(RM) *.def			# Zusätzliche Befehlsdefinitionen
# 	@ $(RM) *.clo			# Optionen von documentclass
	@ $(RM) *.fd			# Zeichensatz-Ordnung (Font Definition)
	@ $(RM) *.tfm			# Zeichensatz-Informationen: Abmessungen, Abstände und Zeichenersatz
	@ $(RM) *.pk			# Zeichensatz-Informationen: Pixelmuster (nur für Druckausgabe oder Preview nötig)
	@ $(RM) *.vf			# virtueller Zeichensatz: Aus welchen Zeichen wird ein Zeichen zusammengesetzt
	@ $(RM) $(NAME).toc		# Table Of Contents (Inhaltsverzeichnis)
	@ $(RM) $(NAME).lot		# List Of Tables (Tabellenverzeichnis)
	@ $(RM) $(NAME).lof		# List Of Figures (Bilderverzeichnis)
	@ $(RM) $(NAME).mtc*		# Minitoc-Paket (Inhaltsverz.  	chapter-level) 
	@ $(RM) $(NAME).mlf*		# Minitoc-Paket (Bilderverz.   	chapter-level)
	@ $(RM) $(NAME).mlt*		# Minitoc-Paket (Tabellenverz. 	chapter-level)
	@ $(RM) $(NAME).slf*		# 				section-level
	@ $(RM) $(NAME).slf*		# 				section-level
	@ $(RM) $(NAME).slt*		# 				section-level
	@ $(RM) $(NAME).plf*		# 				part-level
	@ $(RM) $(NAME).plf*		# 				part-level
	@ $(RM) $(NAME).plt*		# 				part-level
	@ $(RM) $(NAME).idx		# Indexdatei
	@ $(RM) $(NAME).ind		# Indexdatei: Seitenzahlen der Eintäge
	@ $(RM) $(NAME).glo		# Glossary
	@ $(RM) $(NAME).bbl		# BibTeX-Datei
	@ $(RM) $(NAME).blg		# Literaturverzeichnis
	@ $(RM) $(NAME).tpm		# thumbnails im pdf-Dokument
	@ $(RM) $(NAME).ref		# RefTeX-files
	@ $(RM) -r *.prv
	@ $(RM) *.css
	@ $(RM) *.idv
	@ $(RM) *.lg
	@ $(RM) *.xref
	@ $(RM) *.flc
	@ $(RM) *.fls
	@ $(RM) q.log
	@ $(RM) SAVE.fig
	@ $(RM) texput.log
	@ $(RM) _region_.tex
	@ $(RM) _muell_region.tex.tex # AucTeX: latex-buffer Zwischenspeicher
	@ $(RM) $(NAME).4ct
	@ $(RM) $(NAME).4tc
	@ $(RM) $(NAME).xml
	@ $(RM) $(NAME).pdfsync
	@ $(RM) $(NAME).ref
	@ $(RM) -r auto		# Dateien die von RefTeX angelegt werden
	@ $(RM) _muell_region.* # für Emacs interenes kompilieren von Dateien
	@ $(RM) .muell_region.* # für Emacs interenes kompilieren von Dateien
	@ $(RM) _region_.dvi    # für Emacs interenes kompilieren von Dateien
	@ $(RM) _region_.ref    # für Emacs interenes kompilieren von Dateien

.PHONY : cleaner
cleaner: clean
	@ echo "Lösche zusätzlich die Ausgabedateien: pdf, ps, dvi, etc."
	@ $(RM) $(NAME).pdf
	@ $(RM) $(NAME).pdfsync # file used to jump between latex-code and pdf-file
	@ $(RM) $(NAME).ps
	@ $(RM) -r .auctex_info
	@ $(RM) $(NAME).dvi
	@ $(RM) $(NAME)-a5book.ps
	@ $(RM) $(NAME).html
	@ $(RM) $(NAME)2.ps

.PHONY : cleanBackup				# falls eine Datei 'clean' heißt, so verschluckt sich make ansonsten
cleanBackup: cleaner


.PHONY : help				# falls eine Datei 'help' heißt, so verschluckt sich make ansonsten
help:
	@ echo  "Benutzung:"
	@ echo  "   make alleine	erstellt eine dvi-Datei"
	@ echo  "   ps	  		output ist Postscriptdatei"
	@ echo  "   pdf	  		output ist pdf-datei"
	@ echo  "   idx	  		erstelle Indexdatei"
	@ echo  '   index                       "              '
	@ echo  "   mpage	  	Übersicht für Präsentation"
	@ echo  "   thumbpdf	  	output ist pdf-datei mit Thumbnails"
	@ echo  "   bib			BiBTeX wird ausgeführt"
	@ echo  "   2html		HTML-Ausgabe"
	@ echo  "   4html		HTML-Ausgabe (anderes Programm)"
	@ echo  "   a5book		DIN a5 Format"
	@ echo  "   psnup		Doppelseitig"
	@ echo  "   archiv	        siehe tar"
	@ echo  "   tar	  		erstelle Archiv"
	@ echo  "   tar-all  		erstelle Archiv inklusive ps und pdf-Datei"
	@ echo  "   loop	 	hält .dvi-Datei auf neusten Stand"
	@ echo  "   clean  		aufräumen"
	@ echo  "   cleaner  		zusätzlich die Ausgabedateien: pdf, ps, dvi, etc. "
	@ echo  "   2ps                 dvi -> ps ohne neu zu kompilieren"
	@ echo  "   2pdf                ps -> pdf ohne neu zu kompilieren"
	@ echo  "   dvi2pdf	 	Da man mehrere Male das dvi erzeugen sollte (Inhaltsverzeichnis), "
	@ echo  "		   	   macht die Option 2pdf nur die Konvertierung: dvi -> pdf"
	@ echo  "   pslatex		Benutzt pslatex zum kompilieren"
	@ echo  "   pdflatex		Benutzt pdflatex zum kompilieren"
	@ echo  "   reloadxpdf          Startet xpdf neu, falls sich die Datei geändert hat"
	@ echo  "   xpdf 		pdf-Datei betrachten"
	@ echo  "   gv	 		ps-Datei betrachten"
	@ echo  "   pspresent	 	Bildschirmpräsentation von ps-Datei"
	@ echo  "   pdfpresent	 	Bildschirmpräsentation von pdf-Datei"
	@ echo  "   tex			öffnet die Masterdatei"
	@ echo  "   BibDesk		ersetzt ausdrücke in der Literaturdatei: Phys. Rev. Lett. -> PRL, ..."






##################################################
## OHNE Abhängigkeiten (für interene Aufrufe)
##################################################
.PHONY : MakeLatex
MakeLatex:
	@ echo "#############################################"
	@ echo "## LaTeX"
	@ echo "#############################################"
	@ echo "Starte LaTeX ....."
	@ echo "Erstelle die Datei $(NAME).dvi ....."
	@ # mit sed -n '/start/,+N p' werden die N folgenden Linien ausgegeben.
	@ # Damit nicht alles auf Bildschirm angezeigt wird -> Text Filtern:
	@ # weitere Optionen /LaTeX Error/,+20 p' -e "/You can't use /,+20 p" -e "/Extra }, or forgotten/, +20 p"
	@ ### nur Zeilen, die mit einem Ausrufezeichen starten werden ausgegen
	@ ### gebe außerdem alle Zeilen aus die ein .tex enthalten, um nachschauen zu können, in welcher Datei
	@ ###   LaTeX einen Fehler findet
	@ $(LATEX) $(NAME).tex #| $(SED) -n -e '/^!/,+20 p' -e "/\.tex/ p" -e '/^###/p'
	@ echo "LaTeX ohne Fehler beendet."


.PHONY :MakeBibtex
MakeBibtex:
	@ echo "#############################################"
	@ echo "## BibTeX"
	@ echo "#############################################"
	@ # Filtere Text nach Fehlermeldungen:
	@ # Brauche Abfrage nach Warning $(NAME).blg, da Fehler, falls keine Warnings
	@ # touch: legt eine Datei an, falls sie nicht vorhanden ist. Falls eine .tex-Datei keinen
	@ #        \cite-Befehl enthält, so wird von LaTeX keine .aux-Datei angelegt. Dies führt zu Fehlern
	@ #        bei BibTeX. Beachte das $$ im Befehl!!!
	@ echo "Starte BibTeX aus....."
	@ for i in $(TEXFILES);\
	  do \
	    $(TOUCH) $${i%.tex}.aux;\
	  done
	@ $(BIBTEX) $(NAME) | $(GREP) -v "A level-1 auxiliary file:"
	@ echo "BibTeX beendet."
	@ if [ -e $(NAME).blg ] ;\
	  then \
		if ! $(GREP) -q Warning $(NAME).blg ;\
		then \
			echo "Keine Warnungen in BibTeX." ;\
		else \
			$(GREP) Warning $(NAME).blg ;\
		fi ;\
	  fi
	@ if $(GREP) -q "Warning--Warning: pages missing in entry" $(NAME).blg;\
	  then \
		echo "---> Vermutlich hast Du PAGE ansatt PAGES geschreiben" ;\
	  fi ;\
# 	@ if ! $(GREP) -q Citation $(NAME).log || ! $(GREP) -q Warning $(NAME).log ;\
# 	  then \
# 		echo "BibTeX wird nicht benötigt" ;\
# 		if [ -e $(NAME).blg ] ;\
# 		then \
# 			if ! $(GREP) -q Warning $(NAME).blg ;\
# 			then \
# 				echo "Keine Warnungen in BibTeX." ;\
# 			else \
# 				$(GREP) Warning $(NAME).blg ;\
# 			fi ;\
# 		fi ;\
# 		if $(GREP) -q "Warning--Warning: pages missing in entry" $(NAME).blg;\
# 		then \
# 			echo "---> Vermutlich hast Du PAGE ansatt PAGES geschreiben" ;\
# 		fi ;\
# 	  else \
# 		echo "Starte BibTeX aus.....";\
# 		for i in $(TEXFILES);\
# 		do \
# 			$(TOUCH) $${i%.tex}.aux;\
# 		done;\
# 		$(BIBTEX) $(NAME) | $(GREP) -v "A level-1 auxiliary file:" ;\
# 		echo "BibTeX beendet.";\
# 	 fi

.PHONY : MakeWarnings
MakeWarnings:
	@ echo "#############################################"
	@ echo "## LaTeX WARNINGS"
	@ echo "#############################################"
	@ # Gebe alle Warnungen aus:
	@ if ! $(GREP) -q Warning $(NAME).log ;\
	  then \
		echo "Keine Warning vorhanden" ;\
	  else \
		echo "Die folgende Warnungen sind während des kompilierens aufgetreten .....";\
		$(GREP) Warning $(NAME).log ;\
	  fi
	@ if ! $(GREP) -q "! TeX capacity exceeded, sorry" $(NAME).log ;\
	  then \
		echo "Keine Warning vorhanden" ;\
	  else \
		echo "***** ";\
		echo "  TeX hat keine Kapazitäten mehr siehe in $(NAME).log nach:" ;\
		echo "  ! TeX capacity exceeded, sorry" ;\
		echo "***** ";\
	  fi


.PHONY : MakeUndefinesReferences
MakeUndefinesReferences:
	@ echo "############################################"
	@ echo "## Undefined References"
	@ echo "############################################"
	@ if ! $(GREP) -q "LaTeX Warning: Reference" $(NAME).log ;\
	  then \
		echo "Keine undefinierten Referenzen vorhanden" ;\
	  else \
		echo "Die folgende Warnungen sind während des kompilierens aufgetreten .....";\
		$(GREP) "LaTeX Warning: Reference" $(NAME).log ;\
	  fi


.PHONY : MakeIndex
MakeIndex:
	@ echo "Index ist noch nicht implementiert"


.PHONY : MakePSlatex
MakePSlatex:
	@ # mit sed -n '/start/,+N p' werden die N folgenden Linien ausgegeben.
	@ # Damit nicht alles auf Bildschirm angezeigt wird -> Text Filtern:
	@ # weitere Optionen /LaTeX Error/,+20 p' -e "/You can't use /,+20 p" -e "/Extra }, or forgotten/, +20 p"
	@ ### nur Zeilen, die mit einem Ausrufezeichen starten werden ausgegen
	@ ### gebe außerdem alle Zeilen aus die ein .tex enthalten, um nachschauen zu können, in welcher Datei
	@ ###   LaTeX einen Fehler findet
	@ $(PSLATEX) $(NAME).tex #| $(SED) -n -e '/^!/,+20 p' -e "/\.tex/ p"


.PHONY :MakePDFlatex
MakePDFlatex:
	@ if $(GREP) -q psfrag $(TEXFILES); then\
		echo "Ersetzungen in den Bildern mittels psfrag funktioniert nicht.";\
	  fi
# 	@ echo -n "BibTeX funktioniert. (getestet)"; read muell
	@ echo "Starte pdfLaTeX ....."
# 	@ ${MAKE} eps2pdf # erstellt pdfs aus den eps-Dateien
	@ # mit sed -n '/start/,+N p' werden die N folgenden Linien ausgegeben.
	@ # Damit nicht alles auf Bildschirm angezeigt wird -> Text Filtern:
	@ # weitere Optionen /LaTeX Error/,+20 p' -e "/You can't use /,+20 p" -e "/Extra }, or forgotten/, +20 p"
	@ ### nur Zeilen, die mit einem Ausrufezeichen starten werden ausgegen
	@ ### gebe außerdem alle Zeilen aus die ein .tex enthalten, um nachschauen zu können, in welcher Datei
	@ ###   LaTeX einen Fehler findet
	@ $(PDFLATEX) $(NAME).tex #| $(SED) -n -e '/^!/,+20 p' -e "/\.tex/ p"


# In der Latexdatei steht eine Zeile, die 'makedriver' definiert
# \newcommand{makedriver}{...}
# Hier wird getestet, ob diese Option mit dem Aufruf des Makefiles übereinstimmt.
### FUNKTIONIERT NICHT
CHECKLATEX:
	@ echo "##################################################"
	@ echo "##         Check Makedriver Optionen            ##"
	@ echo "##################################################"
	# ich substituiere grep falsch: dies liefert den Rückgabewert echo $?
	@ if [ `grep --count '{\\makedriver}{latex}' $(NAME).tex` -ne 0 ] ; then \
		echo "*** ABBRUCH"; \
		echo "    In $(NAME).tex steht grep --count '\\newcommand{\\makedriver}' $(NAME).tex ";\
		echo "    Schreibe dies um oder benutze die richtige Makefile Option.";\
		echo "    Makefile Option mit: Makefile --help";\
		quit;\
	fi



##################################################
## ???
## Falls diese Dateien noch nicht vorhanden, so soll dass Programm
## nicht abrechen. Deshalb ...
## Dies ist noch unschön und sollte verbessert werden
##################################################
$(INHALTESVERZEICHNISSE) $(BIBTEXFILES):





##########################################################
## Erklärung der Makros
##########################################################
#   $@                  setzt den Befehlsnamen (heißt eigentlich Ziel) ein (Bsp. pdf in LaTeX Makefile)
#   ${NAME:.old=.new}   ersetzt NAME.old durch NAME.new (also Extension wird geändert)
#   $*                  stetzt den Befehlsnamen (=Ziel) ein, aber ohne Suffix (=Endung .c, .o, .tex, ...)
#   $<                  darf nur in Suffixregeln verwendet werden. Falls es wie in .c.o verwendet wird,
#                         so ersetzt es die .o-Datei durch die .c-Datei, falls die letztere neuer ist!!!
#   @ kommando          unterdrückt die Ausgabe des Kommandos auf dem Bildschirm

# Passe darauf auf, dass mit Bash-Befehle mit ";" und "\" zu einer Zeile zusammengefasst werden. Make
#  macht jedes Kommando in einer neuen Subshell, so dass "if" vom Rest getrennt wird -> Unsinn
# Man kann alle Bash-Befehle benutzen, muss aber die Dollarzeichen durch ein zweites schützen
#  also anstatt $ mache $$

